Flexible Operator Embeddings via Deep Learning

Integrating machine learning into the internals of database management systems requires significant feature engineering, a human effort-intensive process to determine the best way to represent the pieces of information that are relevant to a task. In addition to being labor intensive, the process of hand-engineering features must generally be repeated for each data management task, and may make assumptions about the underlying database that are not universally true. We introduce flexible operator embeddings, a deep learning technique for automatically transforming query operators into feature vectors that are useful for a multiple data management tasks and is custom-tailored to the underlying database. Our approach works by taking advantage of an operator's context, resulting in a neural network that quickly transforms sparse representations of query operators into dense, information-rich feature vectors. Experimentally, we show that our flexible operator embeddings perform well across a number of data management tasks, using both synthetic and real-world datasets.

==> background.tex <==
\section{Neural networks background}\label{sec:nn}
Deep neural networks  (DNNs) have a long-ranging history~\cite{universal_approx}, and have recently enjoyed a surge in popularity~\cite{deep_learning}. This section will cover the basics of DNNs and gradient descent, the primary method for training neural networks. A more detailed discussion can be found in~\cite{deep_survey}.

A DNN model is structured in \emph{layers}, where the first layer takes in a vector representing the input data, and each subsequent layer applies some transformation of the previous layer's output. Each layer consists of nodes which receives input data, {multiplies each input by a coefficient (\emph{weight}), sums the result, and passes that sum through an activation function.}
% sums them with a set of coefficients (\emph{weights}), and passes them through an activation function, to produce its output.
The activation function introduces non-linearity, allowing neural networks to represent arbitrary functions~\cite{universal_approx}. Intuitively, activation functions helps the network represent the extent that a particular input value affects the ultimate outcome (e.g., ``is this feature helpful is predicting latency data without error?''), and hence determines whether and to what extent that value progresses further through the network to affect the ultimate outcome (i.e., a node's output is ``activated'' or ``deactivated'').

DNNs end in an \emph{output layer}: a {layer}
% classifier
responsible for mapping the output of the penultimate layer to a prediction. 
DNNs are trained on a dataset, consisting of pairs of \emph{inputs} and \emph{targets}, and aim to learn to accurately map a given input to the correct target. The quality of this mapping is measured by a \emph{loss function}, which quantifies the difference between the neural network's prediction (output) and the ground truth (target). DNNs learn via a process called \emph{gradient descent}, a method that incrementally adjusts the transformation performed by each layer (i.e., the weights), to minimize the loss function. Training a DNN can be seen as a corrective feedback loop, rewarding weights that support correct guesses,  punishing weights that lead to {prediction errors},
% off-predictions
and slowly pushing the loss function towards smaller and smaller values. In the process, the network takes advantage of correlations and patterns in the underlying data, creating new, transformed representations of the data. Simultaneously, the network learns to recognize correlations between relevant features and optimal predictions.
Next, we describe the above using more formal definitions, essential for the introduction of our techniques. 


\subsection{Layers} 
Each layer  in a DNN  is composed of an affine transformation of its input\footnote{Different application domains may use more complex transformations.} and a non-linear \emph{activation function}. Given an input vector $\vec{x}$ of size $n \times 1$, the $i$-th layer of a network can be defined as a function $t_i(\vec{x})$ that provides an output vector of size $m$:% Formally: 
\begin{equation}
\label{eq:affine}
t_i(\vec{x}) = S\left( W_i \times \vec{x} + \vec{b_i} \right) 
\end{equation}
where $S$ is the activation function and $W_i$ are the \emph{weights} for the $i$-th layer, represented by a matrix of size $m \times n$. The bias, $\vec{b_i}$, is an $m \times 1$ vector representing the constant shift of an affine transform. Together, the weights and the biases represent the \emph{parameters} of the neural network model, and control the properties of the transformation performed at each layer. The activation function, $S$, represents some differentiable but non-liner function: popular choices include a sigmoid function or a rectified linear function~\cite{relu}.

Neural network layers are composed together by feeding the output of one layer into the input of the next. For a neural network with $n$ layers, where $\circ$ represents the {function composition operator}, {a neural network} can be defined as:
\begin{equation}
N(\vec{x}) = t_{n} \circ t_{n-1} \circ \dots t_1
\end{equation}
 For example, a two layer neural network $N$ on an input vector $\vec{x}$ could be represented as:
\begin{equation*}
\begin{split}
N(\vec{x})=t_2(t_1(\vec{x})) =S \left(W_2 \times S\left(W_1 \times \vec{x} + \vec{b_1}\right) + \vec{b_2}\right)
\end{split}
\end{equation*}
\subsection{Gradient descent} \label{sec:gd}

The first step to training a neural network $N$ is defining a \emph{loss function}, i.e. a function whose minimization is a suitable criteria for the network to  provide a good prediction.  Let us assume a  set of training input vectors $X$  and a \emph{labeling function} $l(\vec{x})$ that provides the  corresponding target value for each vector $\vec{x} \in X$. For example, if $X$ is a set of vectors representing query plans, $l(\vec{x})$ could be the latency of the query plan represented by the vector $\vec{x}$. The neural network $N$ can be trained to  produce the  target $l(\vec{x})$ when fed $\vec{x}$ by minimizing a loss function~\cite{sgd}.  One popular loss function is $L_2$ loss, or root mean squared error, which can be defined as: 
\begin{equation}
\label{eq:ex_loss}
err(X) = \sqrt{\frac{1}{|X|} \sum_{\vec{x} \in X} \left( N(\vec{x}) - l(\vec{x}) \right)^2}
\end{equation}
Given a loss function and a dataset, the next task is to adjust the weights and biases of the neural network to minimize the loss function. One popular technique for tweaking the weights and biases  is with gradient descent~\cite{sgd}. Here, the  activation function $S$ is chosen to be differentiable so that the loss function can be differentiated with respect to any particular parameter. This allows us to calculate the \emph{gradient}: the derivative of the loss function with respect to an arbitrary parameter ({i.e. a weight in $W_i$ or a bias in $\vec{b}_i$ for some $i$}
  % or bias
). This represents how the loss function is affected by the particular parameter (i.e., if a higher/lower weight/bias leads to higher/lower loss). The derivative of a particular parameter $w$ (i.e., a single element inside of a weight matrix or bias vector) can be written as the following function:
\begin{equation}
\label{eq:gradient}
\nabla_w(err, X) = \frac{\partial err(X)}{\partial w}
\end{equation}
In other words, the gradient of a parameter of the neural network (weights and biases)  is the \emph{derivative of the loss function with respect to this particular parameter.} This gradient can then be evaluated  given the input vectors $X$ and their corresponding target values $l(\cdot)$.

Gradient descent works by adjusting each weight of the neural network independently. The gradient descent algorithm first computes the  gradient (Equation~\ref{eq:gradient}) of a given neural network parameter, $w$. If the gradient is positive, meaning that an increase in this parameter would (locally) lead to a increase in the loss function, the weight $w$ is decreased. If the gradient is negative, meaning that an increase in this parameter would (locally) lead to a decrease in the loss function, the weight $w$ is increased. After adjusting the weight, the algorithm then repeats this procedure for each parameter in the network. This simple procedure is iterated until gradients of all parameters (weight and biases) are relatively flat (i.e., convergence).

In practice, computing the gradient for the entire dataset (i.e., all of input vectors and target values), is prohibitive. Thus, \emph{stochastic} gradient descent instead takes a simple random sample of the input vectors and their corresponding target values and uses these to \emph{estimate} the gradient~\cite{sgd}.

%\input{rnns}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "vldb2019"
%%% End:


